ChatTracer: Large Language Model Powered Real-time Bluetooth Device Tracking System

Large language models (LLMs) have transformed the way we interact with cyber technologies. In this paper, we study the possibility of connecting LLM with wireless sensor networks (WSN). A successful design will not only extend LLM's knowledge landscape to the physical world but also revolutionize human interaction with WSN. To the end, we present ChatTracer, an LLM-powered real-time Bluetooth device tracking system. ChatTracer comprises three key components: an array of Bluetooth sniffing nodes, a database, and a fine-tuned LLM. ChatTracer was designed based on our experimental observation that commercial Apple/Android devices always broadcast hundreds of BLE packets per minute even in their idle status. Its novelties lie in two aspects: i) a reliable and efficient BLE packet grouping algorithm; and ii) an LLM fine-tuning strategy that combines both supervised fine-tuning (SFT) and reinforcement learning with human feedback (RLHF). We have built a prototype of ChatTracer with four sniffing nodes. Experimental results show that ChatTracer not only outperforms existing localization approaches, but also provides an intelligent interface for user interaction.

==> 2_preliminary.tex <==

% It is estimated that 5.9 billion Bluetooth devices will be shipped by the end of 2024 \cite{btmarket}.
% % , with this technology being integrated into nearly every smartphone, laptop, tablet, wearable device, and car \cite{btmarket}. 
% %
% Given that the vast majority of mobile devices have been equipped with Bluetooth, \pname listens to BLE signals from the devices in the proximity to track their locations. 
% Such a BLE-based tracking system will make it possible to track the mobile devices' locations \cite{zhuang2022bluetooth, briggs2022ble, givehchian2022evaluating, zhang2022good} and activities (and thus people's locations and activities) in a \textit{non-invasive} manner \cite{barman2021every, albazrqaoe2016practical, saltaformaggio2016eavesdropping, ai2022blacktooth}. 
% % To design such a system, it is critical to understand the fundamentals, standards, and vendor's implementation of BLE on prevalent devices.
% %
% % In what follows, we first provide preliminaries on BLE signals and protocols, and then present our findings of BLE packets from various devices via extensive measurement. 

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=3.0in]{figures/transceiver.png}
% %     \caption{Bluetooth transceiver architecture.}
% %     \label{fig:transceiver}
% % \end{figure}




% \subsection{Preliminaries on BLE Protocols}


% \textbf{Physical-Layer Parameters:} 
% % Operating within the globally available 2.4 GHz Industrial, Scientific, and Medical (ISM) spectrum band, Bluetooth has become synonymous with short-range wireless data exchange \cite{ghori2020bluetooth}. 
% %
% % Fig.~\ref{fig:transceiver} shows a generic architecture of Bluetooth transceivers. 
% Bluetooth operates on 2.4GHz and mainly uses a Gaussian Frequency Shift Keying (GFSK) modulation scheme for its signal waveform.
% % This modulation ensures the efficient use of bandwidth and reliable data transmission as well as the minimum interference between adjacent channels.  
% %
% It comprises two specifications: Bluetooth Classic (BTC) and Bluetooth Low Energy (BLE) \cite{btspec}. 
% % Both of them operate within the 2.4 GHz ISM band but serve different applications. 
% BTC is typically used for data streaming applications \cite{cominelli2020even}.
% % It is the only one supporting the Advanced Audio Distribution Profile (A2DP) required for audio streaming applications (e.g., Apple CarPlay and Android Auto) and headsets \cite{cominelli2020even}.
% It employs frequency hopping strategies across 79 predefined channels, each 1MHz wide.
% %, to mitigate interference and enhance coexistence with other wireless devices. 
% %
% In contrast, BLE was designed for energy-efficient, short-range data transmission applications.
% %, making it particularly suited for a wide range of battery-powered devices such as wearables, smart home automation systems, and healthcare devices.
% It utilizes 40 channels with 2 MHz spacing, catering to the demands of low-power applications like wearable devices and IoT sensors \cite{jeon2018ble, yang2020beyond, spachos2020ble}. 
% %
% % Both BTC and BLE implement adaptive frequency hopping (AFH) strategies, dynamically selecting channels to optimize signal quality and reduce interference.





% \textbf{BLE Advertisement (Adv) Packets:} 
% Various types of data packets have been defined in the Bluetooth standards to establish and maintain connections as well as facilitate the exchange of data between devices, such as BLE Adv packets, connection request packets, scan response packets, data packets, and control packets.
% %, channel map update packets, and feature exchange packets.
% Among these packets, BLE Adv packets are fundamental to Bluetooth protocol, serving as a mechanism for device discovery, connection initiation, and efficient communication between Bluetooth devices. 
% The Adv Packets provide a means for devices to periodically announce their presence, capabilities, and current status, enabling dynamic and context-aware interactions in diverse Bluetooth-enabled environments.
% Different from data packets that jump across 37 channels, Adv packets are transmitted on three advertising channels.
% The format and data fields of BLE Adv packets have been standardized, providing a structured way to convey information about the advertising device.
% Fig.~\ref{fig:applepkt} shows the format of BLE Adv packets. 

% % \begin{figure}
% % \centering
% % \includegraphics[width=\linewidth]{figures/multi_packet2.pdf}
% % \caption{\label{fig: multi_packet} 
% % One Bluetooth device has multiple BLE advertising addresses for different types of BLE packets.
% % % One Bluetooth device has multiple types of BLE Adv packets, each with a unique advertising address that is changing every 15 minutes.
% % }
% % \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{figures/ble_packet.pdf}

% \caption{The Structure of BLE Adv Packet.}
% \label{fig:applepkt}
% \end{figure}




% % In general, it includes 
% % i) a preamble that helps the Rx device synchronize its clock with the Tx device,
% % ii) a fixed access address that identifies the packet as a BLE packet.
% % %and distinguishes BLE packets from other wireless communication protocols,
% % iii) a protocol data unit (PDU) that carries the payload information about the advertising device for various purposes, 
% % and
% % iv) a cyclic redundancy check (CRC) bit sequence that allows the receiving device to verify the correctness of the received data.




% \textbf{Multiple Advertising Addresses from Single Device:}
% % As shown in Fig.~\ref{fig: multi_packet}, 
% A Bluetooth device typically broadcasts different types of BLE Adv Packets for different purposes (e.g., Proximity Pairing, Handoff, Nearby Action, and Find-My). 
% Different types of BLE Adv Packets have different advertising addresses.
% For every type of BLE Adv Packets, their advertising address changes approximately every 15 minutes due to the addressing randomization mechanism for security reasons. 

 





% % \subsection{Large Language Model}
% % With the advancement of computing capabilities and resources, large language models have attained unprecedented performance in various domains, marking one of the most significant milestones in artificial intelligence and natural language processing. Typically trained on textual data, these models can extend their learning to other modalities like video, audio, and images, enabling them to discern intricate patterns and relationships within diverse datasets. After their initial training, these models can be fine-tuned for specific tasks or domains, empowering them to adapt to specialized applications, including, but not limited to, chatbots, language translation, code generation, and more.




% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\linewidth]{figures/apple_cmmd_rate_active.pdf}
% %     \caption{Measured Apple device BLE broadcast rate.}
% %     \label{fig:apple_ble_rate}
% % \end{figure}




% \subsection{Understand Apple Devices' BLE}
% \label{subsec:apple_ble}


% Decoding the payload of the BLE Adv packets is critical for the design of \pname. 
% In this part, we focus on understanding the BLE Adv Packets from Apple devices. 
% Fig.~\ref{fig:applepkt} shows the BLE Adv frame of Apple devices.
% It carries the Company ID, which is 0x004C for Apple, in its payload, followed by one or multiple Apple Continuity Messages (ACM). 
% In general, we would like to find answers to two questions:
% %
% \textit{(i) How many BLE Adv packets will be broadcast by an Apple device in active (in use) and inactive (not in use) status?} 
% % The more BLE Adv packets an Apple device broadcasts, the more signals \pname can be collected to estimate the location of the device. 
% % This information is critical to evaluate the feasibility and generalizability of \pname. 
% %
% \textit{(ii) What information can we obtain from the BLE Adv payloads (i.e., ACM)?}
% % As we will show, this information will be useful to accelerate the BLE packet grouping for \pname. 
% % It will also be useful for \pname to profile the activities of the device (and thus infer the user's activity).





% Unfortunately, very limited information can be found in the literature or on public websites for those two questions. 
% We thus conduct extensive experiments by using a radio sniffing device to continuously listen to all three Adv channels. 
% The experiments involve 25 different Apple devices and last for 14 days. 
% We collected over 68 million BLE Adv packets from those Apple devices. 
% \textbf{For the first question}, we found that all Apple devices broadcast BLE Adv packets at a surprisingly high rate.
% Fig.~\ref{fig:apple_ble_rate} shows our measurement results. 
% In active status, all 25 Apple devices broadcast more than 273 BLE packets per minute. 
% In inactive (idle, not being used) status, all 25 Apple devices broadcast more than 256 BLE packets per minute. 
% In particular, even if an iPhone has been powered off, it still broadcasts about 50 BLE Adv packets per minute. 
% We guess Apple does so intentionally to increase the user experience of their products and services, such as quick device discovery, seamless data exchange between devices, Nearby services, and Find-My services. 
% The frequent broadcast of BLE Adv packets on Apple devices makes it possible for \pname to track their locations in real-time. 

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\linewidth]{figures/apple_cmmd_rate_both_status2.pdf}
% %     \caption{Apple devices' broadcast rate of BLE Adv packets with specific message type in its payloads when the device is active (top) and inactive (bottom).}
% %     \label{fig:apple_cmmd_rate_both_status}
% % \end{figure}



% \textbf{For the second question}, we found that a sniffing node can profile an Apple device's activity (and thus the user's activity) by decoding the ACMs in its BLE Adv packets.
% %
% As shown in Fig.~\ref{fig:applepkt}, an ACM has two key parts: 
% \textit{type} and \textit{content}. 
% Among the 68 million BLE packets that we collected from 25 different Apple devices, we observed ten ACM types:
% 0x05 (AirDrop),
% 0x07 (Proximity Pairing), 
% 0x08 (Hey Siri),
% 0x09 (AirPlay Target),
% 0x0A (AirPlay Source),
% 0x0B (Magic Switch), 
% 0x0C (Handoff),
% 0x0F (Nearby Action),
% 0x10 (Nearby Info),
% and
% 0x12 (Find My).
% %
% % Fig.~\ref{fig:apple_cmmd_rate_both_status} presents our observed ACM types in terms of their broadcast rate. 
% %
% Intensive measurement shows that different Apple devices broadcast different subsets of ACM types.
% The broadcast of each ACM type is frequent, albeit at different rates. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/apple_ble_rate.pdf}\vspace{-0.25in}
%     \caption{Measured Apple device BLE broadcast rate.} 
%     \label{fig:apple_ble_rate}
% \end{figure}


% By decoding the content in each type of ACM, a sniffing node can profile the Apple device information, including its property (e.g., device model), status (e.g., battery and screen status), and activities (e.g., phone call, Face-Time, video streaming, and gaming).
% For instance, for a BLE packet with ACM type 0x07, content 0x200e means that the device model is ``Airpods Pro;''
% content 0x2b means that the device status is ``Both AirPods in Ear.''
% For a BLE packet with ACM type 0x0F, content 0x2 means that the device model is ``iPhone;'' content 0x0F means that the device status is ``Answered Phone Call.''
% % The information from ACM content can be used to profile the device's activity (thus the user's activity).
% %
% % A natural question is how long it takes for a sniffing node to profile an Apple device
% % (i.e., obtaining all information from one target device). 
% % Fig.~\ref{fig: grouping_time} presents our case studies. 
% % It can be seen that most of devices can be profiled within 2s. 








% % and can be used to identify the device and infer its status and activity. 
% % Through extensive experiments, we decrypt seven CMMD codes as follows:
% % 0x07 is for Proximity Pairing, 
% % 0x09 is for AirPlay Target,
% % 0x0B is for Magic Switch, 
% % 0x0C is for Handoff,
% % 0x0F is for Nearby Action,
% % 0x10 is for Nearby Info,
% % and
% % 0x12 is for Find My.
% % \hz{[where is model info?]}
% % %
% % Fig.~\ref{fig:apple_cmmd_rate_both_status} presents our measurement results of those seven message types on 25 Apple devices when they are in active (being used) and inactive (idle) status. 
% % %
% % It can be seen that different Apple devices broadcast different subset of message types in their BLE packets at different rates. 
% % %
% % \hz{why do we need these codes? why they are useful?}


 






% % \hz{obtain model information of the device.}
 
 


% % In this section, our focus will be on the Apple continuity message, where we will ascertain the feature packet for different Apple devices. As depicted in Table \ref{fig:apple_tablee}, all Apple devices are equipped with the latest firmware and will continuously transmit numerous BLE Advs to enhance the seamless Apple ecosystem, thereby providing a superior user experience. 
% % It is crucial to emphasize that these Advs will be transmitted continuously, regardless of the device's activity status, whether the screen is on or off, or whether specific applications are running or not. This means that the transmission of BLE Advs will remain unaffected as long as Bluetooth is enabled on the device. This setting is highly universal in our daily lives, owing to the widespread popularity and practicality of Bluetooth.


% % \begin{table}
% % \centering
% % \caption{
% % Measured BLE Adv Packets from Different Apple devices in the number of packets per minute.
% % % The variety and quantity of Advs vary across different Apple devices. The number represents the count of each type of Adv per minute, with each type corresponding to the message type in the Apple Continuity Protocol. 
% % % Note: Different activities on Apple devices can lead to the transmission of various Advs. For example, activities like AirPrint and HomeKit, although not as common as other types of Advs, can generate specific ads. In this context, we focus on the most general Advs found on Apple devices.
% % }
% % \includegraphics[width=\linewidth]{apple_tablee.pdf}
% % \label{fig:apple_tablee}
% % \end{table}

% % Referring to Table \ref{fig:other_tablee} and Table \ref{fig:apple_tablee}, we can observe that these devices transmit data very frequently, generating hundreds of packets per minute, even in idle states, with Apple devices being particularly notable in this regard. Transmitting such a high volume of Advs per minute makes it feasible to obtain a sufficient number of packets for tracking, even if the device is within the range of the BLE sniffer for only a few seconds.



 
% % Due to the inherent broadcasting feature of Bluetooth Low Energy, we can receive various BLE packets almost anywhere using a single Software Defined Radio or even our smartphones. Apple Continuity stands out as one of the most universal and fundamental BLE-based protocols in the Apple ecosystem. It facilitates seamless nearby applications such as network sharing, file transferring, and device pairing. These Apple Continuity messages are integrated into the payload of BLE Adv packets, which are periodically broadcasted by all Apple devices as long as they have Bluetooth enabled. However, these protocols have been demonstrated to show that the format and content of Continuity messages can be exploited to fingerprint the type and operating system (OS) version of a device, as well as behaviorally profile users \cite{2019handoff}. Moreover, they can be used for passive tracking, potentially leaking a wide range of personal information \cite{2020discontinued}.
% % As we can effortlessly receive numerous BLE Advs passively, meanwhile, LLM necessitates vast amounts of data for effective training and optimal performance. This piques our curiosity and raises the question: is it feasible to utilize these abundant BLE Advs as real-time data to train the LLM, enabling us to track the behavior or activities of individuals we are interested in?





% % \begin{table}
% % \centering
% % \caption{\label{fig:other_tablee}The number of Advs emitted by different non-Apple devices.}
% % \hz{This table should be used only for android devices. Many more devices are needed.}
% % \includegraphics[width=\linewidth]{other_tablee.pdf}
% % \end{table}







% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/android_BLE_rate.pdf}
%     \caption{Measured Android device BLE broadcast rate.} 
%     \label{fig:android_BLE_rate}
% \end{figure}



% \subsection{Understand Android Devices' BLE}

% \label{subsec:android_ble}

% Unlike Apple devices, Android devices do not transmit many types of BLE Adv packets. 
% Per our measurement, Android devices transmit two types of BLE Adv Packets.
% One carries manufacturer information; the other carries Google's UUID code. 
% %
% We have collected 32 million BLE Adv packets from 23 different Android devices when they are in use and not in use. 
% Fig.~\ref{fig:android_BLE_rate} presents our measurement results. 
% We found that, when being used, those Android devices broadcast more than 235 BLE packets per minute.
% When not being used, those Android devices still broadcast more than 109 BLE packets per minute.
% %
% In addition to Apple and Android devices, some companies may have their own implementations of Bluetooth chipset, such as Sony and Microsoft. 
% % We have also measured the BLE Adv packet rate on a Sony headset (Sony WH-1000XM5). 
% We also conducted experiments to measure their BLE broadcast rate in the condition without active use of the devices. 
% Our measurement shows that a Sony headset (Sony WH-1000XM5) broadcasts BLE Adv packets at 207 packets per minute and a Microsoft Laptop broadcasts at 846. 
% This confirms the widespread availability of BLE Adv packets among mobile devices from different vendors. 
 
% % In the preceding subsection, we elucidated that identifying devices, except for Apple products, is relatively straightforward. All that is needed is to extract the company ID from the manufacturer-specific section of the payload. The number of Advs emitted per minute is illustrated in Table \ref{fig:other_tablee}. 




% % \textcolor{blue}{Given the abundance of BLE Advs everywhere, the initial challenge we must address is differentiating packets originating from various devices. To tackle this issue, we collected and analyzed over 100 million Bluetooth Adv packets over a span of two weeks. These packets were sourced from a diverse range of electronic devices, including iPhone, MacBook, Apple Watch, AirPods, Microsoft Desktop, Samsung Phone, Xiaomi Phone, Google Pixel, and Sony headsets. 
% % }








==> 4_bt_sniffer.tex <==
The purpose of grouping is to identify the source device in the database, if already created, for the newly received BLE packet. 
Since solely using AoA and CFO is not reliable for grouping the packet, we propose a new grouping strategy that combines the physical and payload features of the newly received BLE packet. 
In what follows, we first describe our observations on the time alignment of BLE packets and then present our grouping strategy. 


\subsection{Time Alignment of BLE Packets}

In our experiments, we observed that all BLE packets from one device are well aligned in time. 
Denote $t_j$ as the time moment when the first sample of the $j$th BLE packet is being received (i.e., timestamp in the database).
Denote $\Delta t = |t_j-t_{j'}|$ as the time gap between any two packets from the same Bluetooth device. 
Then, our observation can be written as:
% \begin{equation}
%     \bmod(|t_j - t_{j'}|, 625\mu\mathrm{s})  
%     \approx  \tau_\mathrm{offset}. 
% \end{equation}
\begin{equation}
\Delta t - 
\left\lfloor
\frac{\Delta t}{625\mu\mathrm{s}} 
\right\rceil
\times 
625\mu\mathrm{s}
=  \tau_\mathrm{fix} + \epsilon,
\end{equation}
where $\lfloor\cdot\rceil$ is the rounding operator, $\tau_\mathrm{fix}$ is a fixed value, and $\epsilon$ is an error that may be caused by the device's clock jitters. 



Fig.~\ref{fig:offset} presents the $\epsilon$ distribution of 100 million BLE packets from 25 different Apple devices and 23 different Android devices.
It can be seen that the time error $\epsilon$ of Apple BLE packets ranges from 0 to 6$\mu$s.
This means that, if \pname solely uses time alignment for Apple packet grouping, the grouping error probability is about 6/625$\approx$1\%.
It can also be seen that the time error $\epsilon$ of Android BLE packets ranges from 0 to 9$\mu$s.
If \pname solely uses time alignment for Android packet grouping, the grouping error probability is about 9/625$\approx$1.5\%.
%
Therefore, to achieve reliable packet grouping, \pname combines all physical and payload features for packet grouping. 

% The time alignment will be used as another PHY-layer feature, along with AoA, CFO and RSS, to determine the source device of a newly-received BLE packet.



% To verify this observation, we conduct experiments on a number of Apple and Android Bluetooth devices. 


\begin{figure}
\centering
\includegraphics[width=\linewidth]{results/offset.pdf} 
\caption{Error $\epsilon$ distribution of time alignment between packets from the same device.}
\label{fig:offset}
\end{figure}








\subsection{Our Grouping Strategy}

% Before describing the algorithm, we first introduce notation. 
Referring to the database entries in Fig.~\ref{fig:systemarc}, for a specific scenario, we denote $\mathcal{D} = \{d_1, d_2, \ldots, d_I\}$ as the set of devices already in the database.
%, where $I$ is the number of devices.
Denote $\mathcal{P}_i = \{p_{i,1}, p_{i,2}, \ldots, p_{i,n_i}\}$ as the set of packet entries in the database under Device $d_i$.
%, where $n_i$ is the number of packet entries under this device thus far. 
Our grouping strategy comprises three steps in sequential order.


$\bullet$
\textbf{Step I: Adv\_address matching.} 
We check the adv\_address from the new BLE packet, and search it in the database. 
If we find that the same adv\_address has appeared under Device $d_i$ in the database, we insert this new BLE packet into the entries of Device $d_i$. 
We are done with the grouping of this packet. 
This is because adv\_address, albeit generated randomly, has 6 bytes and can be regarded as unique for identity in practice. 
If adv\_address is not found in the database, there are two possibilities: 
i) this is a new adv\_address from an existing device due to address randomization;
ii) this adv\_address is from a new device. 
In this case, the algorithm runs into the next step. 

$\bullet$
\textbf{Step II: Payload feature matching.}  
In this step, the algorithm uses the payload features in the BLE packet to exclude those impossible devices in the database, aiming at reducing the search space and search computation.
Specifically, we select a subset of features: 
$\mathcal{F}_\mathrm{fix} = \{\mathrm{vendor}, \mathrm{model}, \mathrm{color}\}$.
These features are fixed and will never change for a device. 
Denote $\mathcal{D}_\mathrm{match}$ as a subset of $\mathcal{D}$ whose $\mathcal{F}_\mathrm{fix}$ features match with those carried by the new BLE packet (if any). 
%
% If $\mathcal{D}_\mathrm{match}$ has only one Device ID, the new BLE packet is inserted into database under this device. 
% The algorithm terminates. 
% %
If $\mathcal{D}_\mathrm{match}$ is empty, a new Device ID is created in the database and this BLE packet is inserted into the database under this device.
The algorithm terminates.
%
If $\mathcal{D}_\mathrm{match}$ has one or multiple devices, the algorithm proceeds. 
 
$\bullet$
\textbf{Step III: Feature weighted scoring.} 
In this step, \pname uses the combination of physical-layer features (CFO, AoA, RSS) to determine the device source of a packet.
Specifically, denote $p$ as the BLE packet under consideration. 
Denote $p'$ as the latest BLE packet under Device $d_i$ in the database.
Then, for each $d_i \in \mathcal{D}_\mathrm{match}$, we calculate its score by:
\begin{align}
    S_i = &
    W_\mathrm{TS}\frac{[TS(p) \!\!-\!\! TS(p')]\%625\mu s \!\!-\!\! \tau_\mathrm{fix}}{TS_\mathrm{thre}}
    +
    W_\mathrm{AoA}\frac{AoA(p) \!\!-\!\! AoA(p')}{AoA_\mathrm{thre}} 
    \nonumber \\
    &
    +
    W_\mathrm{CFO}\frac{CFO(p) - CFO(p')}{CFO_\mathrm{thre}}
    +
    W_\mathrm{RSS}\frac{RSS(p) - RSS(p')}{RSS_\mathrm{thre}},
    \nonumber
\end{align}
\!\!where $TS(\cdot)$, $AoA(\cdot)$, $CFO(\cdot)$ and $RSS(\cdot)$ denote the timestamp, AoA, CFO and RSS values of the BLE packet. 
$TS_\mathrm{thre}$, $AoA_\mathrm{thre}$, $CFO_\mathrm{thre}$ and $RSS_\mathrm{thre}$ are empirically predefined threshold values.
$W_\mathrm{TS}$, $W_\mathrm{AoA}$, $W_\mathrm{CFO}$ and $W_\mathrm{RSS}$ are empirically predefined weights for those features. 
Then, \pname calculates 
$i^* = \arg\max_{d_i \in \mathcal{D}_\mathrm{match}} \{S_i\}$.
If $S_{i^*} \leq S_\mathrm{thre}$, where $S_\mathrm{thre}$ is a predefined score threshold, the BLE packet is inserted into the database under Device $d_{i^*}$;
otherwise, a new Device ID is created in the database for this BLE packet. 

\begin{comment}
    

\subsection{Grouping Performance}

\qw {Add table. Not sure if we should put it here or in evaluation.}
\qw{
The result of packet grouping with different feature setting and device manufactures are shown in Table \ref{table:pkt_grouping}. The accuracy of packet grouping does not increase significantly because with the time alignment feature, our algorithm already can achieve high accuracy. To accelerate processing time, we utilize other features like AoA, CFO, and RSS. By incorporating AoA, the processing time decreases by 46.16\% and 44.28\% for Apple and Android devices, respectively. This reduction is because, within a short time period, the AoA values of packets from the same device are typically stable, which helps the algorithm exclude some packets to accelerate the process. After combining CFO, there is no noticeable impact on Apple devices, due to the similarity of CFO among them, while it speeds up the process for Android devices due to their diversity. Lastly, RSS further helps to decrease the grouping time for both Apple and Android devices.
}
\input{packet_grouping_table}
\end{comment}

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{figures/possibility2.pdf}
% \caption{The probability of linking BLE advertisements varies across different recording time periods and devices.}
% \hz{not cited.}
% \label{fig: grouping_time}
% \end{figure}


% Therefore, we employ a weighted formula of all those features to score each device in $\mathcal{D}$. 
% If the minimum score is ...
% \hz{complete it.}

 


% In the previous subsection, we identified the types of packets transmitted by various devices. Distinguishing non-Apple devices is straightforward, as each device transmits advertisements through a single advertising address. However, the challenge arises with Apple devices, as depicted in Table \ref{fig:apple_tablee}. A single Apple device emits multiple types of advertisements, each utilizing a distinct advertising address. 
% Moreover, different devices might transmit the same type of BLE advertisement packet, especially ones like Find My, Nearby Info, and Nearby Action.
% These kind of BLE packets are transmitted by almost all Apple devices. 


% Given that each advertisement type contains information about the device, which is linked to its owner, it becomes crucial to differentiate packets emitted by the same Apple device. This distinction is essential not only for accurately constructing individual profiles but also for improving tracking performance, as one individual may use multiple devices.

\begin{comment}
    

These devices encompass different operating systems, chipsets, and hardware drivers. Along with these devices, we explore whether only the BLE packets emitted by specific device models and/or device status can be grouped by our algorithm.

We start by assessing the time required to link BLE advertisements with different brands and numbers of devices in our controlled environment.

Considering the fact that all Bluetooth packets emitted by a single device, whether Bluetooth Classic (BTC) or Bluetooth Low Energy (BLE), are driven by a common oscillator, there is a fundamental synchronization. Bluetooth Classic packets are consistently synchronized to 625 $\mu s$, and Bluetooth Low Energy packets can be linked to Bluetooth Classic packets by measuring the time difference between them \cite{sp2021}. However, the transmission rate of BTC packets is generally lower than that of BLE packets when the devices are not in use, which could pose challenges in tracking inactive devices. As shown in Table \ref{fig:apple_tablee}, we observe that we can assign a specific feature packet to each type of Apple device, as certain packets are only emitted by specific devices, or we can obtain model information from the payload of the packet. For example, only the MacBook emits AirPlay Target messages, while the Apple Watch emits Magic Switch messages. Additionally, we can obtain the AirPods model from the Proximity Pairing packet. Based on this observation, we are intuitively exploring the possibility of calculating the time difference between the feature packet and other types of packets from a single Apple device to distinguish them from packets emitted by other devices.

To determine whether packets are emitted by a single Apple device, it is necessary to identify the unique feature packet of a device and quantify the time difference between other packets and their respective nearest feature packets. Although BLE advertisements are synchronized with the advertising event and not aligned to 625 $\mu s$ like BTC, they are inherently interconnected \cite{sp2021}. On the other hand, our Bluetooth sniffer system can calculate the CFO, RSSI, and AoA of each packet. Packets from the same devices are expected to exhibit nearly identical values for these parameters within a concise timeframe. Therefore, we will also consider these parameters to identify packets emitted by the same device. We outline our methodology for a brief period of advertisements as follows:

\begin{enumerate}
    \item Record \& decode IQ samples received by SDRs, and calculate CFOs, RSSIs, and AoAs for all Bluetooth packets. 
    \item Extract $	\left( M+N \right) \times C $ BLE advertisements along with their corresponding normalized CFOs, RSSIs, AoAs within a specified time period, denoted as $\left\{ BLE_{i,j}^{F}, CFO_{i,j}^{F}, RSSI_{i,j}^{F}, AoA_{i,j}^{F}  \right\}$, $i \in [0, M-1]$,  $j \in [0, C-1]$ and $\left\{ BLE_{k,l}^{O}, CFO_{k,l}^{O}, RSSI_{k,l}^{O}, AoA_{k,l}^{O}  \right\}$, $k \in [0, N-1]$,  $l \in [0, C-1]$. Here, $M$ represents the number of different BLE feature advertisements, $N$ represents the number of different BLE non-feature advertisements and $C$ represents the number of different advertising channel indices.
    \item For each combination of $BLE_{i,j}^{F}$ and $BLE_{k,l}^{O}$, calculate the time difference (modulo 625$\mu s$) and indicator distance $\left\{ D_{i,j,k,l}^{(h)}  \right\}$, $h \in [0, H-1]$, for each of H non-feature packet $BLE_{i,j}^{O}$ and the nearest $BLE_{k,l}^{F}$ feature packets and then driven the combination's score as:
    \begin{itemize}
        \item $S_{i,j,k,l} = \sqrt{\frac{1}{L}\sum_{h=0}^{H-1}(D_{i,j,k,l}^{(h)})^2}$ if $h=0$
        \item $S_{i,j,k,l} = \sqrt{\frac{1}{L}\sum_{h=0}^{H-1}(D_{i,j,k,l}^{(h)}-mode({D_{i,j,k,l}}))^2}$ if $h>0$
    \end{itemize}

    \item Determine $BLE_{i,j}^{F}$ and $BLE_{k,l}^{O}$ are emitted by the same device if ($S_{i,j,k,l} < \bar{S}$ and $H_l > \bar{H}$), where $\bar{S}$ and $\bar{H}$ are the thresholds for the score and the number of advertisements, respectively.
\end{enumerate}

In this scenario, the goal is to identify all BLE advertisements, including both feature and non-feature advertisements, transmitted by M BLE devices. Specific applications running on the BLE devices are not necessary for our analysis.

First, we record and decode packets emitted by Bluetooth devices over a specified period. We then extract Bluetooth Low Energy advertisements and obtain details such as advertising addresses, timestamps, CFOs, RSSIs, and AoAs for all packets. These packets are categorized into two datasets: $M$ feature BLE advertisements denoted as $BLE_{i}^{F}$ and $N$ non-feature BLE advertisements denoted as $BLE_{k}^{O}$.

Next, we analyze the correlation between each pair of feature BLE advertisements and other BLE advertisements. To achieve this, we calculate the differences in timestamps (modulo 625$\mu s$), CFOs, RSSIs, and AoAs between each non-feature advertisement and the nearest feature advertisement. To account for clock drift in Bluetooth devices, we search for the nearest feature packet within a predefined time window. If no feature packet is found within the window, the advertisements are discarded. Based on our observations, excluding timestamps and CFOs provides reliable results in most cases. Combining RSSI and AoA enhances linkage performance in scenarios where the target is static. Consequently, we gather $H$ pairs of BLE feature advertisements $BLE_{i,j}^{F}$ and non-feature advertisements $BLE_{k,l}^{O}$,  calculating the distance between them to create a vector of $H$ elements $\left\{ D_{i,j,k,l}^{(h)}  \right\}$, where $h \in [0, H-1]$ represents each non-feature packet on each channel and its nearest corresponding feature packet.

Finally, we quantify the correlation by computing a score $S_{i,j,k,l} = \sqrt{\frac{1}{L}\sum_{h=0}^{H-1}(D_{i,j,k,l}^{(h)})^2}$ as the Root-Mean-Square-Error of the packet distances for each pair of $BLE_{i,j}^{F}$ and $BLE_{k,l}^{O}$. A lower score indicates a higher likelihood of correlation. The linkage thresholds $\bar{S}$ and $\bar{H}$ are determined based on our experimental results, where $\bar{S}$ represents the score threshold and $\bar{H}$is the minimum number of matches required to make a decision. A match is established when $S_{i,j,k,l} < \bar{S}$ and $H_l > \bar{H}$), signifying that the advertisements are emitted by the same Bluetooth device.

\end{comment}

% \subsection{Device Activity Profiling}

==> 5_llm.tex <==

% In this section, we provide a comprehensive overview of the motivation behind and the numerous advantages of utilizing LLMs to implement an efficient localization system. Furthermore, we introduce the meticulously designed LLM integrated with our cutting-edge Bluetooth sniffer technology. This integration empowers our system to seamlessly localize and track individuals in real time, ensuring unparalleled accuracy and efficiency in diverse applications.



% \subsection{Data Collection and Processing}
% The data used to fine-tune and test our LLM is sourced from our custom-designed and highly efficient Bluetooth sniffer system, as detailed in the preceding section. Since the performance of LLMs is significantly influenced by the diversity and quality of the dataset, we carefully collect data across various scenarios over a sufficient duration to eliminate accidental interference. 



% \subsection{Fine-tuning}
% In this section, we will describe the process of fine-tuning the LLM, encompassing supervised fine-tuning, reward modeling, and RLHF.


\pname employs Mistral-7B as its base LLM. 
The tasks of Mistral-7B include:
i) understand the queries in English text from end users;
ii) infer the location of a device based on its BLE packet features in the database;
iii) generate the trajectory of a device based on its location history;
and
iv) provide the status and activity information of a specific device. 
%
Task~(i) does not need fine-tuning the model, because an LLM has already been pre-trained for understanding and generating human-like text. 
Task~(iv) does not need fine-tuning the model, either.
This is because this task does not involve much inference. 
The model simply extracts the device status and activity information from the database (see Fig.~\ref{fig:systemarc}), rephrases and/or reorganizes it, and reports the results to end users. 
%
The fine-tuning is mainly for Tasks (ii) and (iii), which involve reasoning, nonlinear regression, denoising, and removing outliers in both spatial and temporal domains. 



We employ two techniques to fine-tune the Mistral-7B model: 
SFT and RLHF. 
The former focuses on improving the LLM's localization accuracy, while the latter focuses on enhancing the LLM's overall performance. 
Fig.~\ref{fig:finetune} shows the diagram of our fine-tuning strategy. 
We describe them below. 







\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/LLM_training.pdf} 
\caption{\pname's fine-tuning diagram.}
\label{fig:finetune}
\end{figure}



\subsection{Supervised Fine-Tuning (SFT)}
\label{subsec:sft}

SFT comprises three steps:
data collection, data annotation, and prompting-based model fine-tuning. 

\noindent
\textbf{Data Collection:}
Our data collection campaign lasted for more than six months. 
We collected data in five scenarios: 
lab, building hallway, apartment, shopping mall, and university library.
In each scenario, we capture the BLE Adv packets from our own smart devices (35 Apple devices and 25 Android devices).
We extracted their physical and payload features and stored them in the format as shown in Fig.~\ref{fig:systemarc}. 
For each device, we record their locations (two-dimensional coordinates) and activities (e.g., watching videos, making phone calls, and listening to music) over time, which are used as ground-truth labels for SFT.
The collected feature and location/activity data are linked together through their timestamps.
The data collected at one location for one device is called one data sample. 
In total, we collected 60,000 data samples for the SFT of Mistral-7B. 



% During data collection, our participants use their devices under controlled conditions. It's important to note that one individual might handle multiple devices. For instance, someone might use AirPods, which connect to their mobile phones for listening to music or watching streaming videos. Our participants follow instructions to stand, sit in various locations, or walk along predefined trajectories. We utilize a laser to measure and determine the ground-truth locations.



\begin{table}
\footnotesize
\centering
\caption{A template sample of SFT annotation.
The parts marked by red fonts are variables that should be instantiated by the collected data samples.}
\label{tab:SFT_table}
\begin{tabular}{lp{7.0cm}}
\hline
% $\bullet$ 
\textbf{Prompt:}
& 
We are in scenario \textcolor{red}{$S$}. 
Its area size is \textcolor{red}{$X$} meter by \textcolor{red}{$Y$} meter. 
In this scenario, \textcolor{red}{$N$} Bluetooth sniffing nodes have been deployed at coordinates: \textcolor{red}{${(A_1, B_1), (A_2, B_2),\ldots,(A_N, B_N)}$}.
The coordinate axis's origin is located at the northwest corner. 
In this area, multiple individuals carry Bluetooth devices and engage in different activities.
%
We have gathered the BLE Adv packets as follows: 
\textcolor{red}{$\mathcal{P}_1$}, \textcolor{red}{$\mathcal{P}_2$}, \textcolor{red}{$\ldots$}, \textcolor{red}{$\mathcal{P}_K$}.
Please calculate the most recent locations of these \textcolor{red}{$K$} devices based on the above information.  \\
%
% the Angle of Arrival (AoA) and Received Signal Strength (RSS) for these devices, presented as follows: $\{\{dev_1, AoA_{11}, AoA_{12} ... AoA_{1n}; RSSI_{11}, RSSI_{12} ... $ $ RSSI_{1n}\}, \{dev_2, AoA_{21}, AoA_{22} ... AoA_{2n}; RSSI_{21}, RSSI_{22} ... RSSI_{2n}\}, ...\}$. (Note: AoA is measured as 0 degrees when the signal is received from the north orientation, increasing counterclockwise up to 360 degrees).
% Please calculate the locations of these \textcolor{red}{$N$} devices based on the above information.  \\
% \hline
\textbf{Response:}\!\!\!\!
& 
Certainly. Based on the information you provided, the $K$ devices are likely located at:
\textcolor{red}{$(X_1, Y_1)$}, \textcolor{red}{$(X_2, Y_2)$}, \textcolor{red}{$\ldots$}, \textcolor{red}{$(X_K, Y_K)$}. 
Among these \textcolor{red}{$K$} devices, \textcolor{red}{$K_1$} devices are Apple devices and \textcolor{red}{$K_2$} devices are Android devices.\\

\hline\hline
% $\bullet$ 
\textbf{Prompt:} 
& 
Please generate the trajectory of all the devices.
\\

% \hline
\textbf{Response:}\!\!\!\!
& 
Certainly. 
The trajectories of the $K$ devices are given as below.\ \ 
\makecell{
Device \textcolor{red}{$1$}: \textcolor{red}{$(X_{11}, Y_{11})$}, \textcolor{red}{$(X_{12}, Y_{12})$}, \textcolor{red}{$\ldots$} \\
Device \textcolor{red}{$2$}: \textcolor{red}{$(X_{11}, Y_{11})$}, \textcolor{red}{$(X_{12}, Y_{12})$}, \textcolor{red}{$\ldots$} \\
\textcolor{red}{$\cdots$}\\
Device \textcolor{red}{$K$}: \textcolor{red}{$(X_{11}, Y_{11})$}, \textcolor{red}{$(X_{12}, Y_{12})$}, \textcolor{red}{$\ldots$}\\
}
\\
\hline
\hline
% $\bullet$ 

\textbf{Prompt:} 
& In this case, provide me with more details about these devices. \\
% \hline

\textbf{Response:}\!\!\!\!
& Certainly. 
It appears that $K_3$ devices are stationary, and $K_4$ devices are moving. 
\textcolor{red}{$K_5$} devices are MacBook Pro;
\textcolor{red}{$K_6$} devices are iPhone; 
\textcolor{red}{$K_7$} devices are Samsung phones. 
\textcolor{red}{$K_8$} Apple devices are watching video;
\textcolor{red}{$K_9$} Apple devices are on phone call;
\textcolor{red}{$K_{10}$} Apple devices are with Airpods.
\\
\hline
\end{tabular}
\end{table}


\noindent
\textbf{Data Annotation:}
A naive approach to fine-tuning the model is using the feature data as input and the location/activity data as output. 
This approach is efficient for training an application-specific model (e.g., transformer) but appears to be inefficient for training LLM. 
To enhance the training efficiency, we created 15 contextual templates, as exemplified by Table~\ref{tab:SFT_table}. 
In this contextual template instance, we created the prompt and response by mimicking a real use case.
The parts marked by red fonts are variables, which are instantiated by the data samples from our collected dataset described above. 



The contextual templates, after being instantiated by the collected data samples, are used to fine-tune the Mistral-7B model.
%
During SFT, the base model is fine-tuned for three epochs using cross-entropy loss on the output conditioned on the input. 
Our training process uses a cosine learning rate schedule with 200 warm-up steps, an initial learning rate of $2.0\times 10^{-5}$, a batch size of 32, and a weight decay of 0.05. 
%
The low-rank adaptation (LoRA) \cite{hu2021lora} technique was used for SFT to expedite the fine-tuning process while maintaining the memory requirements.


\textbf{Few-shot Chain-of-Thought (CoT) Reasoning:}
In addition to standard prompting, we employ Few-Shot-CoT prompting \cite{wei2022chain, kojima2022large} to improve \pname's ability to perform complex reasoning. 
%
Table~\ref{tab:CoT_table} shows an example of Few-Shot-CoT prompting.
It teaches \pname to solve problems by mimicking the step-by-step reasoning process of the prompt.
%  
% CoT prompts, consisting of intermediate reasoning steps, aim 
In our experiments, the results from ablation studies will show the effectiveness of Few-Shot-CoT in enhancing \pname's generalizability, leading to better localization accuracy in unseen scenes. 


\begin{table}
\scriptsize
\centering
\caption{An example of Few-Shot-CoT prompting.}\vspace{-0.10in}
\label{tab:CoT_table}
\begin{tabular}{lp{6.75cm}}
\hline
% $\bullet$ 
\textbf{\makecell{Model\\input}}\!\!\!\!\!\!\!
& 
\textbf{Q:} How many people are in the current apartment?\smallskip

\textbf{A:} First, we analyze the data on electronic devices present in the apartment. We have 4 Apple devices and 2 Android devices, making a total of 6 devices.
Upon examining the proximity of these devices, it's noted that a pair of AirPods, an iPhone, and an Apple Watch are very close to each other, suggesting that they belong to the same person due to their approximate 7 cm distance.
Another set of devices, including a pair of AirPods and a Samsung Phone, are about 10 cm apart, indicating another individual's possessions.
The remaining device, a Xiaomi Phone, given the distances between device pairs (3.78 meters, 1.92 meters apart), suggests it belongs to a third individual.
Considering the distribution and proximity of devices, we can infer that there are likely 3 individuals present in the apartment. 
So the answer is 3.\smallskip

\textbf{Q:} The total number of visitors to the dining hall will increase by 50\% tomorrow compared to today. We know the number of visitors to the food station PANGEA will increase by 150\%. Please calculate the number of visitors that will go to the other food stations, excluding PANGEA. 
\\
\textbf{\makecell{Model\\output}}\!\!\!\!
& 
\textbf{A:} Start with the total number of visitors to the dining hall today, which is 1294.
The number of visitors to PANGEA today is 36.
To find the total number of visitors tomorrow, we calculate $1294 \times (1 + 0.5) = 1941$. This accounts for a 50\% increase.
For the PANGEA station, a 150\% increase is expected, so we calculate $36 \times (1 + 1.5) = 90$ visitors for tomorrow.
To find the number of visitors to the other food stations, excluding PANGEA, we subtract the number of visitors to PANGEA from the total number of visitors tomorrow: 1941 - 90 = 1851.
So the answer is 1851.

\\\hline
\end{tabular}
\end{table}



% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{figures/CoT11.pdf}
% \caption{\pname's chain-of-thought example.}
% \label{fig:CoT}
% \end{figure}


% To enhance localization accuracy and leverage the capabilities of the LLM, we integrate contextual information with the original data. Specifically, we manually assess the quality of measured data, such as AoAs and RSSIs, which are susceptible to environmental influences. For example, certain areas in the shopping mall have a Line-of-Sight to some Software-Defined Radios (SDRs), ensuring relatively accurate AoAs. However, in Non-line-of-sight situations, where signals may be obstructed by walls or equipment, the measured AoAs are inaccurate. We annotate such cases and selectively mask or ignore specific measured data, enhancing localization accuracy. This level of nuanced decision-making is challenging for other deep learning models but is facilitated by the human-like reasoning ability of the LLM.

% Following data processing and screening, we eventually construct a customized Bluetooth device localization dataset comprising approximately 60,000 prompt-response pairs. All the data underwent rigorous de-identification procedures to safeguard the privacy of users.






% \textbf{Training Format????.}
% In the realm of supervised fine-tuning, we adopted a highly effective and efficient technique known as low-rank adaptation (LoRA) to fine-tune ChatTracer. 
% Since there is no public dataset available for us to fine-tune the model, we manually annotate several thousand examples of high-quality SFT data, the template of the conversations are as illustrated in Table \ref{tab: SFT_tablee}.

\subsection{Reinforcement Learning with Human Feedback (RLHF)}

% While SFT aims to improve the localization and tracking performance of the LLM, RLHF aims to enhance its overall performance including user experience, accuracy, robustness, and usability. 

SFT appears to be effective in understanding domain-specific knowledge and enhancing the reasoning capability of LLM for our localization/tracking tasks. 
However, during our tests, we observed frequent instances of refused answers, performance degradation in unseen scenarios, and LLM hallucinations. 
To address these issues, we employ RLHF for fine-tuning the LLM, with the aim of improving its accuracy, generalizability, and answer rate while reducing the rate of its hallucinations. 
%
Our RLHF procedure comprises two steps:
\textit{training a reward model (RM)} 
and
\textit{reinforcement learning}.


\textbf{Reward Model and Its Training:}
As shown by Step 2 in Fig.~\ref{fig:finetune}, we employ an RM and train it through human annotation to evaluate the output of \pname (after being fine-tuned in \S\ref{subsec:sft}).
Specifically, the RM takes a response generated by \pname and its corresponding prompt, including contexts from previous turns, as inputs.
It then outputs a scalar score indicating the quality of the generated response.
%
For the training of this RM, we asked seven people to manually rank the responses generated by \pname.
%based on the annotation criteria provided in Table~\ref{tab:annotations}. 
%
To train the RM, we initialize its parameters using the SFT model from the previous step, with the final unembedding layer removed. 
We train the RM for two epochs with a batch size of 64 and a learning rate
$10^{-5}$, using the AdamW optimizer.
%
The RM is trained to minimize the following \mbox{loss function \cite{ouyang2022training}:}
%
\begin{equation}
\mathcal{L}_\mathrm{RM}(\theta) = -\frac{1}{\binom{K}{2}}\mathbb{E}_{(x,y_p,y_r)\in \mathcal{A}}
\big[\log(\sigma(r_{\theta}(x,y_p)-r_{\theta}(x,y_r)))\big],
\nonumber
\end{equation}
where $K$ is the number of the responses to the prompt,  $\theta$ is the RM parameters, $r_{\theta}(\cdot,\cdot)$ denotes the output of the RM. 
$\mathbb{E}[\cdot]$ denotes the expectation.
$\mathcal{A} = \{(x, y_p, y_r)\}$ denotes  the manually sorted dataset, where $x$ is the input, $y_p$ and $y_r$ are the outputs marked as ``better" and ``worse."

% \qw{
% For the training process, we initialize the reward model with the SFT model from previous step with the final unembedding layer removed. 
% We train our reward model for 2 epochs with a batch size of 64 and a learning rate
% of 1e-5, using the AdamW optimizer.
% }


% \input{annotations}

\textbf{Reinforcement Learning:}
After being trained, the RM is used to improve the overall performance of \pname's LLM through reinforcement learning, as illustrated by Step 3 in Fig.~\ref{fig:finetune}.
%
\begin{comment}
    

We configure the number of model responses, denoted as $K$, to be 4, and employ the trained RM to automatically assess the generated responses.
\end{comment}
%
Throughout the reinforcement learning process, we adopt the Proximal Policy Optimization (PPO) algorithm \cite{schulman2017proximal} to direct the model's updates by leveraging the evaluation results from the RM. 
% PPO stands out as an efficient reinforcement learning algorithm, leveraging the evaluation results from the RM to direct the model's updates. 
The PPO objective function is defined as follows:
\begin{equation}
\mathcal{L}_\mathrm{RL}(\phi) = -\mathbb{E}_{x \sim D_{RL}, y \sim \pi_{\phi}^{RL} (y|x)}
\big[r_{\theta}(x,y)-\beta \cdot KL(x,y)\big],
\nonumber
\end{equation}
where $D_{RL}$ corresponds to the prompt distribution, $\pi_{\phi}^{RL}(y|x)$ denotes the learned RL policy, $\pi ^ {SFT}$ is initialized with the SFT model. $KL(x,y) = \log(\pi _ \phi ^ {RL} (y|x) / \pi ^ {SFT} (y|x)) $ is the Kullback–Leibler divergence to penalize large deviation of $\pi _ \phi ^ {RL}$ from the initial SFT policy $\pi ^ {SFT}$\!, and $\beta$ is is the hyper-parameter to control the scale of the KL penalty.

 
During the RL training, we performed four PPO epochs. We employ the AdamW optimizer with $\beta _ 1 = 0.9$, $\beta _ 2 = 0.95$, and $\beta _ 1 = 5\times10^{-9}$. The KL coefficient $\beta$ is set to 0.05; the weight decay is 0.1; and the learning rate is $1.0\times 10^{-5}$. In each PPO iteration, we set a batch size to 32 and the PPO clip ratio to 0.2.
%
Through the RLHF process, the domain knowledge and reasoning capability of human people can be transferred to the LLM for the localization and tracking tasks.


\begin{comment}
\newpage

We ask annotators to assess model-generated dialogues across these dimensions in descending priority.

In the end, we utilize the annotated ranking data to train the reward model (RM). This model takes a response generated by the system and its corresponding prompt, including contexts from previous turns, as inputs. It then outputs a scalar score indicating the quality, encompassing factors like accuracy and safety, of the generated response. 




By utilizing these response scores as rewards, we can optimize ChatTracer during Reinforcement Learning with Human Feedback (RLHF). This optimization process leads to better alignment with human preferences and enhances the overall accuracy and safety of the system.

The reward model (RM) incorporates a linear layer into the original model, with a dialogue pair $(x, y)$ as input, and produces a scalar reward value that reflects the quality of the input dialogue. The objective of RM is to minimize the following loss function:
\begin{equation}
L(\theta) = -E_{(x,y_h,y_l)\in D}[log\sigma(r_{\theta}(x,y_h)-r_{\theta}(x,y_l)] \nonumber
\end{equation}
where $r_{\theta}$ denotes the reward model, and $\theta$ is generated parameter. $E_{(x,y_h,y_l)\in D}$ denotes the expectation over each tuple $(x, y_h, y_l)$ in the manually sorted dataset $D$, where $x$ is the input, and $y_h$, $y_l$ are the outputs marked as "better"
and "worse".

\end{comment}



==> 5_llm_backup1.tex <==

In this section, we provide a comprehensive overview of the motivation behind and the numerous advantages of utilizing LLMs to implement an efficient localization system. Furthermore, we introduce the meticulously designed large language model integrated with our cutting-edge Bluetooth sniffer technology. This integration empowers our system to seamlessly localize and track individuals in real-time, ensuring unparalleled accuracy and efficiency in diverse applications.


\subsection{Why LLM}
In light of the myriad potent deep-learning models available today, adept at tackling localization challenges, it is imperative to elucidate the essentiality and significance of integrating Large Language Models (LLMs) into localization systems.

\begin{itemize}
\item Precision Redefined. Imagine a world where every inch of indoor space is meticulously mapped, where locating an object or a person is as precise as pinpointing a star in the night sky. LLMs, powered by their ability to comprehend intricate patterns, enhance the accuracy of indoor localization by processing and interpreting the complex data derived from the AoAs and RSSIs. Additionally, they can integrate additional contextual information, such as the layout of the buildings or historical location data. This contextual information further enhances the accuracy of location estimates.
\item Humanizing Technology. Indoor localization with LLMs is more than just technology; it's a bridge between the digital and physical realms. By harnessing the power of natural language understanding, this approach makes technology accessible and intuitive. People can interact with the system using natural language queries, making the user experience seamless and empowering everyone, regardless of their technical expertise, to harness the benefits of precise indoor positioning.
\item Adaptability to New Data. LLMs can undergo continuous refinement through the infusion of fresh ground truth data. As increasingly precise location information becomes accessible, the model dynamically adapts and refines its accuracy, ensuring a perpetual evolution toward unparalleled precision. This adaptive nature not only guarantees accuracy in the present but also signifies a commitment to relentless improvement, making it an invaluable investment for the future.

\end{itemize}


\subsection{Data Collection and Processing}
The data used to fine-tune and test our Large Language Model is sourced from our custom-designed and highly efficient Bluetooth sniffer system, as detailed in the preceding section. Since the performance of Large Language Models is significantly influenced by the diversity and quality of the dataset, we carefully collect data across various scenarios over a sufficient duration to eliminate accidental interference. Specifically, we gather data in our lab, the hallway of the school building, the authors' apartment, the shopping mall, and the university library.

In each scenario, we capture BLE advertisements and calculate the RSSIs, CFOs, and AoAs emitted by electronic devices, such as mobile phones, laptops, headsets, and smart wearables. Simultaneously, we gather and record the status of these devices. This information enables us to infer the activities of the device owners, as we can distinguish between BLE advertisements from the same device. During data collection, our participants used their devices under controlled conditions. It's important to note that one individual might handle multiple devices. For instance, someone might use AirPods, which connect to their mobile phones for listening to music or watching streaming videos. Our participants follow instructions to stand, sit in various locations, or walk along predefined trajectories. We utilize a laser to measure and determine the ground-truth locations.

To enhance localization accuracy and leverage the capabilities of the Large Language Model, we integrate contextual information with the original data. Specifically, we manually assess the quality of measured data, such as AoAs and RSSIs, which are susceptible to environmental influences. For example, certain areas in the shopping mall have a Line-of-Sight to some Software-Defined Radios (SDRs), ensuring relatively accurate AoAs. However, in Non-line-of-sight situations, where signals may be obstructed by walls or equipment, the measured AoAs are inaccurate. We annotate such cases and selectively mask or ignore specific measured data, enhancing localization accuracy. This level of nuanced decision-making is challenging for other deep learning models but is facilitated by the human-like reasoning ability of the LLM.

Following data processing and screening, we eventually constructed a customized Bluetooth device localization dataset comprising approximately 60,000 prompt-response pairs. All the data underwent rigorous de-identification procedures to safeguard the privacy of users.

% \subsection{Fine-tuning}
% In this section, we will describe the process of fine-tuning the LLM, encompassing supervised fine-tuning, reward modeling, and RLHF.

\subsection{Supervised Fine-Tuning}


In the development of our cutting-edge Bluetooth device tracking system, ChatTracer, we harnessed the capabilities of the Mistral-7B model. The Mistral-7B is a potent 7.3 billion-parameter language model that represents a significant advancement in the capabilities of large language models (LLMs). It has consistently outperformed the 13 billion-parameter Llama 2 model across all tasks and surpasses the 34 billion-parameter Llama 1 on numerous benchmarks. In the realm of supervised fine-tuning, we adopted a highly effective and efficient technique known as low-rank adaptation (LoRA) to fine-tune ChatTracer. 

Since there is no public dataset available for us to fine-tune the model, we manually annotate several thousand examples of high-quality SFT data, the template of the conversations are as illustrated in Table \ref{tab: SFT_tablee}.

\begin{table}
\scriptsize
\centering
\caption{SFT annotation}\label{tab: SFT_tablee}
\begin{tabular}{lp{6.9cm}}
\hline
% $\bullet$ 
Prompt: & Now, we find ourselves in scenario X. In this environment, there are N Software Defined Radios (SDRs) deployed at specific coordinates ${(A_1, B_1), (A_2, B_2), ...(A_n, B_n)}$ (with the coordinate axis's origin located at the northwest corner). Within this space, multiple individuals may carry various Bluetooth devices, engaging in different activities. We have gathered the Angle of Arrival (AoA) and Received Signal Strength Indicator (RSSI) for these devices, presented as follows: $\{\{dev_1, AoA_{11}, AoA_{12} ... AoA_{1n}; RSSI_{11}, RSSI_{12} ... $ $ RSSI_{1n}\}, \{dev_2, AoA_{21}, AoA_{22} ... AoA_{2n}; RSSI_{21},$  $ RSSI_{22} ... RSSI_{2n}\}, ...\}$.(Note: AoA is measured as 0 degrees when the signal is received from the north orientation, increasing counterclockwise up to 360 degrees). Your task is to calculate the localizations of these devices based on the provided information. Please note that the area size is $C * D$. \\
% \hline
 Response: & Certainly. Depending on the scenario and the Angle of Arrivals (AoAs) and Received Signal Strength Indicators (RSSIs) you've provided for these devices, we can calculate the localization of each device using the following format: $\{\{dev_1, (X_1, Y_1)\}, \{dev_2, (X_2, Y_2)\}, ...\}$. In total, there are N devices, with P of them being Apple devices and Q being Android devices. \\
\hline
% $\bullet$ 
Prompt: & Based on the localization of these devices, generate the trajectory sequence for them. Please take into account the status, activities of these devices, and the scenario to ensure the results are reasonable. \\

% \hline
 Response: & Certainly, I can assist with this. Taking into account the environment and the status of these devices, I will generate trajectories for you: $\{\{dev_1, (X_{11}, Y_{11}), (X_{12}, Y_{12}) ...\}, \{dev_2, (X_{21}, Y_{21}), $ $ (X_{22}, Y_{22}) ...\}, ...\}$. \\
\hline
% $\bullet$ 

Prompt: & In this case, is there any other information you can provide for me? \\
% \hline

 Response: & Certainly. Analyzing all the information, it appears that two individuals are stationary, utilizing their MacBooks alongside their iPhones. Additionally, one individual is employing an iPhone with AirPods to watch videos, another using an iPhone with AirPods for a phone call, and one individual using a Samsung device. \\
\hline
\end{tabular}
\end{table}

\subsection{Reinforcement Learning with Human Feedback (RLHF)}
While SFT can provide LLM localization and dialogue capabilities, the model might still produce inaccurate, untruthful, or unfriendly responses, potentially leading to negative consequences in various practical applications. To address this issue, we adopt RLHF, a model training procedure applied to a fine-tuned language model, aiming to better align the model's behavior with human preferences and instructions. As pioneers in the application of RLHF in localization LLM, we established a refined ranking annotation rule, which covers three dimensions——Safety, Accuracy, Fluency——an nine specific abilities as shown in Table \ref{tab:annotation_tablee}. We ask annotators to assess model-generated dialogues across these dimensions in descending priority.

In the end, we utilize the annotated ranking data to train the reward model (RM). This model takes a response generated by the system and its corresponding prompt, including contexts from previous turns, as inputs. It then outputs a scalar score indicating the quality, encompassing factors like accuracy and safety, of the generated response. By utilizing these response scores as rewards, we can optimize ChatTracer during Reinforcement Learning with Human Feedback (RLHF). This optimization process leads to better alignment with human preferences and enhances the overall accuracy and safety of the system.

The reward model (RM) incorporates a linear layer into the original model, with a dialogue pair $(x, y)$ as input, and produces a scalar reward value that reflects the quality of the input dialogue. The objective of RM is to minimize the following loss function:

\begin{equation}
L(\theta) = -E_{(x,y_h,y_l)\in D}[log\sigma(r_{\theta}(x,y_h)-r_{\theta}(x,y_l)] \nonumber
\end{equation}
where $r_{\theta}$ denotes the reward model, and $\theta$ is generated parameter. $E_{(x,y_h,y_l)\in D}$ denotes the expectation over each tuple $(x, y_h, y_l)$ in the manually sorted dataset $D$, where $x$ is the input, and $y_h$, $y_l$ are the outputs marked as "better"
and "worse".

To guarantee the model's safety, we meticulously adjust erroneous responses to phrases such as "I'm sorry, I don't know..." This proactive approach significantly heightens the model's awareness of its limitations and capabilities. Throughout the reinforcement learning process, we adopt the Proximal Policy Optimization (PPO) algorithm. PPO stands out as an efficient reinforcement learning algorithm, leveraging the evaluation results from the reward model to direct the model's updates. This strategic utilization further refines the model’s performance, ensuring it closely mirrors the expertise of human professionals.
\begin{table}
\centering
\caption{\label{fig:annotation_tablee}Annotation criteria.}
\includegraphics[width=\linewidth]{figures/annotations.pdf}
\end{table}


==> 8_related_work.tex <==
\textbf{Large Language Model:}
LLMs, exemplified by ChatGPT and GPT-4, have showcased remarkable advancements. 
However, OpenAI has chosen not to divulge its training methodologies or weights. 
As a result, the research community has turned its attention towards open-source LLMs such as
LLaMA \cite{touvron2023llama}, Vicuna \cite{chiang2023vicuna}, and Mistral \cite{jiang2023mistral}.
These alternatives have significantly piqued the interest of researchers.
%
% LLMs such as ChatGPT and GPT-4 have demonstrated remarkable accomplishments, ushering in a new era in artificial intelligence. These models undergo extensive training on vast corpora, equipped with contextualized embeddings that adeptly capture intricate linguistic patterns. Nevertheless, OpenAI has chosen not to disclose their training methodologies or weights, necessitating the research community to turn to open-source LLMs like LLaMA \cite{touvron2023llama}, Vicuna \cite{chiang2023vicuna}, and Mistral \cite{jiang2023mistral}, which have significantly piqued the interest of researchers.
Fine-tuning LLMs emerges as a crucial strategy for customizing these generalized models to suit specific tasks. 
These tasks span diverse fields, including medicine \cite{singhal2023large, wu2023pmc, wang2023huatuo, abd2023large} to multimodality \cite{ye2023mplug, lyu2023macaw, han2023imagebind, hu2023bliva}, 
and autonomous driving \cite{chen2023driving, cui2023receive, sha2023languagempc, xu2023drivegpt4, cui2023drive}.
%
% The RLHF strategy emerges as a powerful tool for fine-tuning LLMs, enabling significant improvements in their performance \cite{christiano2017deep}. 
% The combination of supervised fine-tuning with RLHF has proven effective in tackling issues concerning factuality, toxicity, and helpfulness. These issues cannot be sufficiently addressed through mere scale-ups of LLMs.
%
While LLMs have been used in many fields, they have not been studied with WSNs. 
\textit{Our work differs from existing literature by creating a new application of LLMs and demonstrating the application in realistic scenarios. }




\input{llm_ablation_table1}



% The RLHF strategy emerges as a potent tool for fine-tuning LLMs, facilitating substantial enhancements in their performance \cite{christiano2017deep}. Combining instruction fine-tuning with RLHF has proven effective in addressing issues related to factuality, toxicity, and helpfulness that cannot be adequately resolved through mere scale-ups of LLMs \cite{ouyang2022training}.

% However, a notable gap exists in the literature that revolves around the seamless integration of Language Models (LLMs) with cyber-physical systems. Our proposal seeks to bridge this gap by tapping into the remarkable capabilities of LLMs, aiming to reshape the communication landscape within cyber-physical systems. The crux of our proposition lies in empowering LLMs to adeptly leverage real-time data, a crucial facet that can propel them towards continuous refinement and broadening of their functionalities. This, in turn, holds the potential to elevate the overall quality of services provided to end-users, establishing a novel frontier in the symbiotic relationship between language models and cyber-physical systems.


% \noindent
\textbf{Bluetooth Localization:} 
Bluetooth-based indoor localization has gained significant attention in recent years due to its advantages such as low cost, low power consumption, and widespread availability. 
A common approach for Bluetooth-based indoor localization is to utilize the RSS of BLE beacons for distance estimation. 
Trilateration algorithms are then used to estimate the position of a target device, as demonstrated by the studies in \cite{chen2017locating, peng2016iterative, gleason2018crowdsourcing, phutcharoen2020accuracy}.
%
An alternative strategy for Bluetooth-based indoor localization utilizes the AoA of BLE signals. 
This method calculates phase differences from synchronized antenna arrays to determine the direction, followed by applying triangulation algorithms for position estimation \cite{su2023single, ayyalasomayajula2018bloc, gu2021tyrloc, cominelli2019dead}.
%
\textit{\pname is the first one using LLM for localization, and it demonstrates a superior performance over existing approaches. }

\begin{comment}
\textbf{Bluetooth Device Identification.} 
The broadcast nature of BLE devices exposes users to privacy risks, as investigations into Apple's BLE Continuity protocol have shown \cite{cominelli2020even, barman2021every}. Through reverse engineering, significant data leaks from Apple devices' advertisement packets were uncovered, allowing for potential device identification \cite{martin2019handoff, celosia2020discontinued}. Yet, the challenge arises as a single device can emit various packet types and different devices may simultaneously send identical packets, complicating origin differentiation. CFO could aid in identification and tracking \cite{givehchian2022evaluating}, but its effectiveness is tempered by sensitivity to temperature and commonality among devices from the same manufacturer. Research \cite{ludant2021linking} has shown linking BLE advertisement packets to BT packets aids in long-term tracking, although BT packets' infrequent transmission, especially from idle devices, hampers data collection in dynamic environments. Our novel packet grouping algorithm surpasses previous methods by efficiently combining physical and MAC-layer features for Bluetooth device identification.
\end{comment}

% Bluetooth-based indoor localization has garnered significant attention in recent years owing to its advantages, including low cost, low power consumption, and widespread availability. A prevalent approach for Bluetooth-based indoor localization involves utilizing the received signal strength (RSS) of Bluetooth Low Energy (BLE) beacons to gauge distance. Trilateration algorithms are then applied to estimate the position of a target device, as indicated by various studies \cite{chen2017locating, peng2016iterative, gleason2018crowdsourcing, phutcharoen2020accuracy}. An alternative strategy for Bluetooth-based indoor localization employs the angle of arrival (AOA) of BLE signals. This is achieved by calculating phase differences from synchronized antenna arrays to determine the direction, followed by the application of triangulation algorithms for position estimation, as suggested by several studies \cite{su2023single, ayyalasomayajula2018bloc, gu2021tyrloc, cominelli2019dead}.

% However, existing localization systems fall short of providing accurate and robust localization capabilities, particularly in handling ambiguity and inaccuracies. For instance, some angles or RSSIs provided are not accurate, and the system cannot process this information contextually, such as integrating additional contextual information like the layout of the target area or historical location data. Moreover, integration with conversational systems that are capable of seamlessly managing both user requests and localization tasks within a unified framework, has yet to be achieved.

% Our proposed system, ChatTracer, addresses these limitations, offering a comprehensive solution that seamlessly combines accurate and robust localization capabilities with the ability to process ambiguous, inaccurate, and unstructured data. Notably, ChatTracer ensures adaptability by facilitating continuous upgrades through fine-tuning with fresh data, ensuring its perpetual relevance and effectiveness.

==> annotations.tex <==

\begin{table}[]
\centering
 \caption{Annotation criteria.}
 \label{tab:annotations}
 \hz{not cited.} \qw{looks it has been cited below this table}
 \scalebox{0.7}{
\begin{tabular}{|c|c|l|}
\hline
\textbf{Dimension}  & \textbf{Capability}& \textbf{Definition}  \\ \hline
\multirow{3}{*}{Accuracy}   & Positional Precision   & \begin{tabular}[l]{@{}l@{}}Ensure that the estimated location is as close as\\ possible to the actual physical location.\end{tabular}\\ \cline{2-3} 
& \begin{tabular}[l]{@{}l@{}}Consistency Across\\ Environments\end{tabular}  & \begin{tabular}[l]{@{}l@{}}Provide accurate location estimation across various\\ settings, accounting for factors such as diverse room\\ layouts and obstacles.\end{tabular} \\ \cline{2-3} 
& Temporal Consistency   & \begin{tabular}[l]{@{}l@{}}Maintain accuracy even as the Bluetooth signal\\ environment evolves over time.\end{tabular}  \\ \hline
\multirow{3}{*}{Robustness} & \begin{tabular}[l]{@{}l@{}}Sniffing Node\\ Density Adaptability\end{tabular}   & \begin{tabular}[l]{@{}l@{}}Capable of providing accurate localization even in\\ areas with a sparse distribution of sniffing nodes.\end{tabular} \\ \cline{2-3} 
& Noise Tolerance& \begin{tabular}[l]{@{}l@{}}Capable of handling external factors that may\\ introduce inaccuracies in localization, such as signal\\ noise, interference, or variations.\end{tabular} \\ \cline{2-3} 
& \begin{tabular}[l]{@{}l@{}}Dynamic Environment\\ Adaptation\end{tabular}   & \begin{tabular}[l]{@{}l@{}}Resilience and swift adaptation to dynamic indoor\\ conditions.\end{tabular}  \\ \hline
\multirow{3}{*}{Usability}  & \begin{tabular}[l]{@{}l@{}}User-Friendly\\ Interaction\end{tabular}& \begin{tabular}[l]{@{}l@{}}Ensure the response is easily understandable and \\ actionable, making it accessible to non-expert users.\end{tabular}\\ \cline{2-3} 
& \begin{tabular}[l]{@{}l@{}}Adaptability to\\ Varying User Queries\end{tabular} & Capable of handling a variety of user queries.   \\ \cline{2-3} 
& \begin{tabular}[l]{@{}l@{}}Real-Time\\ Performance\end{tabular}& \begin{tabular}[l]{@{}l@{}}Ensure timely and accurate information for users\\ relying on the system.\end{tabular}\\ \hline
\end{tabular}

}

\end{table}

==> llm_ablation_table.tex <==


\begin{table}[]
\centering
\scriptsize
\caption{Ablation studies of RLHF and CoT.} 
\label{tab:llm_ablation}
\begin{tabular}{l|cc|cc}
\hline
\multirow{2}{*}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ Performance metric}    & \multicolumn{2}{l|}{~~~~~\ \ \ \ \ \ \ \ \ \ \ SFT} & \multicolumn{2}{l}{\ \ \ \ \ \ SFT+RLHF} \\ \cline{2-5} 
& \!\!w/o CoT\!\!     & w/~ CoT      & \!\!w/o CoT\!\!        & w/~ CoT         \\ \hline
\begin{tabular}[c]{@{}l@{}}Median loc. error in fine-tuned scenes\end{tabular} & 0.85m       & 0.67m      & 0.73m          & 0.59m         \\ \hline
\begin{tabular}[c]{@{}l@{}}Median loc. error in unseen scenes \end{tabular}     & 1.03m       & 0.88m      & 0.81m          & 0.65m         \\ \hline
Hallucinations rate                    & 8.9\%       & 8.1\%      & 4.7\%          & 4.2\%         \\ \hline
Answer rate                            & 96.8\%      & 97.0\%     & 99.0\%         & 99.1\%        \\ \hline
\end{tabular} 
\end{table}

==> llm_ablation_table1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\footnotesize
\centering
\caption{\pname with different input information.} 
\label{tab:llm_ablation1}
\begin{tabular}{l|llll}
\hline
Information               & \multicolumn{4}{l}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ Choice} \\ \hline
AoA + RSS                 & \ding{52}     & \ding{52}    & \ding{52}    & \ding{52}    \\
Device model              & \ding{56}     & \ding{52}    & \ding{52}    & \ding{52}    \\
Device activities             & \ding{56}     & \ding{56}    & \ding{52}    & \ding{52}    \\
Environment layout         & \ding{56}     & \ding{56}    & \ding{56}    & \ding{52}    \\ \hline
Median localization error &   1.03m    &  1m    &   0.92m   &  0.66m    \\
Hallucination rate       &   6.3\%    &   5.3\%   &   5\%   &    4.5\%  \\
Answer rate          &    97.9\%   &  98.5\%    &   98.6\%   &     99\%
\\\hline
\end{tabular}
\end{table}

==> llm_ablation_tablee.tex <==
\begin{table}[]
\centering
 \caption{Performance camparison between \pname with and without RLHF.}\label{tab:llm_ablation}
\begin{tabular}{l|llll}
Performance metric                                & \multicolumn{2}{l}{Mistral + SFT} & \multicolumn{2}{l}{Mistral + SFT + RLHF} \\ \hline
With CoT                                          &                 &                 &                     &                    \\
Without CoT                                       &                 &                 &                     &                    \\ \hline
Median localization error in fine-tuned scenarios &                 &                 &                     &                    \\
Median localization error  in unseen scenarios    &                 &                 &                     &                    \\
Hallucinations rate                               &                 &                 &                     &                    \\
Answer rate                                       &                 &                 &                     &                   
\end{tabular}
\end{table}

==> packet_grouping_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Accuracy \& time cost with different feature settings and manufactures.}
\label{table:pkt_grouping}
\begin{tabular}{|c|cccc|c|c|}
\hline
\multirow{2}{*}{}        & \multicolumn{4}{c|}{Features used}                                                  & \multirow{2}{*}{Accuracy} & \multirow{2}{*}{Time (s)} \\ \cline{2-5}
& \multicolumn{1}{c|}{TS} & \multicolumn{1}{c|}{AoA} & \multicolumn{1}{c|}{CFO} & RSS &                           &                       \\ \hline
\multirow{4}{*}{Apple}   & \multicolumn{1}{c|}{\ding{52}}  & \multicolumn{1}{c|}{\ding{56}}   & \multicolumn{1}{c|}{\ding{56}}   & \ding{56}   &     99.26\%                      &        3.3682               \\ \cline{2-7} 
& \multicolumn{1}{c|}{\ding{52}}  & \multicolumn{1}{c|}{\ding{52}}   & \multicolumn{1}{c|}{\ding{56}}   & \ding{56}   &           99.31\%                &         1.8135              \\ \cline{2-7} 
& \multicolumn{1}{c|}{\ding{52}}  & \multicolumn{1}{c|}{\ding{52}}   & \multicolumn{1}{c|}{\ding{52}}   & \ding{56}   &           99.46\%                &         1.6371              \\ \cline{2-7} 
& \multicolumn{1}{c|}{\ding{52}}  & \multicolumn{1}{c|}{\ding{52}}   & \multicolumn{1}{c|}{\ding{52}}   & \ding{52}   &              99.83\%            &         1.1315              \\ \hline
\multirow{4}{*}{Android} & \multicolumn{1}{c|}{\ding{52}}  & \multicolumn{1}{c|}{\ding{56}}   & \multicolumn{1}{c|}{\ding{56}}   & \ding{56}   &       98.85\%                    &     4.8517                  \\ \cline{2-7} 
& \multicolumn{1}{c|}{\ding{52}}  & \multicolumn{1}{c|}{\ding{52}}   & \multicolumn{1}{c|}{\ding{56}}   & \ding{56}   &              98.93\%             &      2.7032                 \\ \cline{2-7} 
& \multicolumn{1}{c|}{\ding{52}}  & \multicolumn{1}{c|}{\ding{52}}   & \multicolumn{1}{c|}{\ding{52}}   & \ding{56}   &               99.39\%            &       1.9158                \\ \cline{2-7} 
& \multicolumn{1}{c|}{\ding{52}}  & \multicolumn{1}{c|}{\ding{52}}   & \multicolumn{1}{c|}{\ding{52}}   & \ding{52}   &               99.62\%            &        1.5335              \\ \hline


\end{tabular}
\end{table}

==> status_table.tex <==
\begin{table*}[]
\centering
 \caption{Linkability in sitting and walking scenarios.}\label{tab:link_tablee}
\begin{tabular}{|c|ccccc|ccccc|}
\hline
Status & \multicolumn{5}{c|}{Sitting}  & \multicolumn{5}{c|}{Walking}  \\ \hline
Device & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Samsung\\ S23U\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Xiaomi\\ 11 Lite\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}iPhone 15\\ Pro Max\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Apple Watch \\ Ultra 2\end{tabular}} & \begin{tabular}[c]{@{}l@{}}AirPods \\ Pro 2\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Samsung\\ S23U\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Xiaomi\\ 11 Lite\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}iPhone 15\\ Pro Max\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Apple Watch \\ Ultra 2\end{tabular}} & \begin{tabular}[c]{@{}l@{}}AirPods \\ Pro 2\end{tabular} \\ \hline
1s  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& \\ \hline
5s& \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& \\ \hline
10s  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{}& \\ \hline
\end{tabular}
\end{table*}
